Enhancing nuclear cross-section predictions with deep learning: the DINo algorithm

Accurate modeling of nuclear reaction cross-sections is crucial for applications such as hadron therapy, radiation protection, and nuclear reactor design. Despite continuous advancements in nuclear physics, significant discrepancies persist between experimental data and theoretical models such as TENDL, and ENDF/B. These deviations introduce uncertainties in Monte Carlo simulations widely used in nuclear physics and medical applications. In this work, DINo (Deep learning Intelligence for Nuclear reactiOns) is introduced as a deep learning-based algorithm designed to improve cross-section predictions by learning correlations between charge-changing and total cross-sections. Trained on the TENDL-2021 dataset and validated against experimental data from the EXFOR database, DINo demonstrates a significant improvement in predictive accuracy over conventional nuclear models. The results show that DINo systematically achieves lower chi2 values compared to TENDL-2021 across multiple isotopes, particularly for proton-induced reactions on a 12C target. Specifically, for 11C production, DINo reduces the discrepancy with experimental data by \sim 28\% compared to TENDL-2021. Additionally, DINo provides improved predictions for other relevant isotopes produced, such as 4He, 6Li, 9Be, and 10B, which play a crucial role in modeling nuclear fragmentation processes. By leveraging neural networks, DINo offers fast cross-section predictions, making it a promising complementary tool for nuclear reaction modeling. However, the algorithm's performance evaluation is sensitive to the availability of experimental data, with increased uncertainty in sparsely measured energy ranges. Future work will focus on refining the model through data augmentation, expanding its applicability to other reaction channels, and integrating it into Monte Carlo transport codes for real-time nuclear data processing.

==> name.tex <==
\section{Results}
The analysis will focus on comparing DINo's predictions with the established TENDL model. As an example, the $^{11}$C product cross-sections will be explored, and the global results for all product cross-sections will be shown after. This choice of charge-changing product was made due to the extensive data available for this cross-section in the EXFOR database, and thus permits to develop and better test our DNN algorithm.\\

To compare the DINo's prediction to the TENDL model one, the $\chi^2$ values will be computed, which can be expressed as :
\begin{equation}
    \chi^2=\sum\frac{(predicted-expected)^2}{expected}
\end{equation}

For each DINo \(\chi^2\) that will be given, the algorithm will be launched 100 times in order to have a reliable mean value and error associated, defined as the standard deviation.

The \(\chi^2\) statistic is a measure used to evaluate the goodness of fit between the predicted and expected values. It assesses whether there is a significant difference between the two sets of values, enabling a comparison of the efficiency of the two models. A lower \(\chi^2\) value indicates a better fit of the model to the experimental data, meaning the predictions are more accurate.

\subsection{Detailed study of $^{11}$C product}
Figure \ref{fig:TENDLvsData_C11} presents the total cross-section and $^{11}$C product cross-section for incident protons on a $^{12}$C target as a function of incident energy comparison between TENDL21 model and experimental data.
\begin{figure*}
\begin{center}
\includegraphics[scale=0.7]{ModelvsData_tot_C11.pdf}
\caption{\label{fig:TENDLvsData_C11} Total cross-section for incident protons on a $^{12}$C target as a function of incident energy alongside with $^{11}$C product cross-section: TENDL21 model predictions compared to experimental data.}
\end{center}
\end{figure*}

The $\chi^2$ estimation concerning the TENDL21 model total cross-section prediction compared to experimental data is of 7.2 $\pm$ 1.1.


Figure \ref{fig:total-cross-sections_test} presents an iteration example of the algorithm tested on the model values. The challenge in deep learning algorithms is that it needs to learn enough to be able to predict results, but not so much that it only replicates the model it was trained on.

\begin{figure*}[htbp]
\begin{center}
\includegraphics[scale=0.7]{AI_prediction_test.pdf}
\caption{\label{fig:total-cross-sections_test} Algorithm test on total cross-section for incident protons on a $^{12}$C target as a function of incident energy alongside: TENDL model results and DINo predictions.}
\end{center}
\end{figure*}

Figure \ref{fig:total-cross-sections} presents the predicted experimental total cross-section values by DINo alongside TENDL model values and the experimental ones. This comparison is important for understanding how well DINo performs in predicting total cross-sections compared to existing models. Notably, within the energy range relevant for particle therapy (above 50 MeV), the predictions generated by the DINo model demonstrate significantly higher accordance to experiment data than those from the TENDL21 model.

\begin{figure*}[htbp]
\begin{center}
\includegraphics[scale=0.6]{C11_predictions.pdf}
\caption{\label{fig:total-cross-sections} Total cross-section for incident protons on a $^{12}$C target as a function of incident energy: TENDL model results and DINo predictions compared to experimental data.}
\end{center}
\end{figure*}

The effectiveness of DINo predictions is further analyzed in Figure \ref{fig:dino-tendl-comparison}, which compares total cross-sections for incident protons on a $^{12}$C target between TENDL model results, DINo predictions, and experimental data. The predicted values from the model and the AI algorithm are plotted as a function of the experimental data values, for each incident energy. The black linear function represents the perfect case where the prediction is equal to the experimental value. The closer the points are from this line, the better the predictions are. 

\begin{figure}[htbp]
    \centering
    \includegraphics[width=0.8\textwidth]{IAvsDatavsModel.pdf}
    \caption{$^{11}$C product cross-sections and total cross-section for incident protons on a $^{12}$C target: TENDL model results and DINo predictions compared to experimental data.}
    \label{fig:dino-tendl-comparison}
\end{figure}

The $\chi^2$ values provide a quantitative measure of compatibility between the experimental data and the predictions. Notably, the $\chi^2$ value between the experimental data and DINo predictions are reported as 5.2$\pm$1.0.
% $2.9 \pm 0.6$, showcasing a superior fit compared to the $\chi^2$ value of $4.5 \pm 1.0$ for the TENDL model.

The results demonstrate that the deep learning algorithm DINo exhibits enhanced predictive capabilities for total cross-sections compared to the TENDL model for which the $\chi^2$ value is 7.2 $\pm$ 1.1. 

Even under the least favorable conditions, when DINo exhibits its lowest performance (indicated by a $\chi^2$ value of 6.1), it still matches the best performance of the TENDL model. In optimal scenarios, DINo outperforms the TENDL model by a factor of almost 2 (1.98), showcasing its potential for accurate predictions in nuclear physics applications.


\subsection{Tests with other products}
Following the evaluation of the $^{11}$C isotope, additional tests were performed on other isotopic products produced via proton-carbon nuclear reactions. The aim was to validate the robustness and versatility of the DINo algorithm across different isotopes and to ensure its predictive accuracy was not limited to a single case. 

When studying the fragmentation of protons on $^{12}$C, the products of interest are those that are most likely to be produced in carbon ion therapy and have significant biological impacts. Here are the key products to focus on:
\begin{itemize}
    \item \textbf{$^4$He}: alpha particles, are significant due to their high LET, which can contribute to the therapeutic effect but also to potential side effects. 
    \item \textbf{$^6$Li}: Lithium isotopes are important to consider because they can result from the breakup of carbon nuclei and have specific biological impacts.
    \item \textbf{$^9$Be}: Beryllium isotopes are less common but still relevant in understanding fragmentation patterns and dose calculations.
    \item \textbf{$^{10}$B }: Boron isotopes are produced in fragmentation and are of interest, especially considering boron neutron capture therapy (BNCT) applications.
\end{itemize}

These choices ensure comprehensive modeling of relevant nuclear interactions, leveraging extensive data availability in TENDL-21.

Table \ref{tab:chi2} presents the \(\chi^2\) values comparing the experimental charge-changing cross sections to the model predictions for various isotopes relevant to carbon ion therapy. 

\begin{table*}[!hbt]
\begin{center}
	\begin{tabular}{|l||c|c|}
	\hline
    Isotope & DINo's prediction \(\chi^2\) & TENDL21 Model \(\chi^2\) \\ \hline
	\hline
    Helium-4 ($^4$He) & 2.2 $\pm$ 0.4 & 3.0 $\pm$ 0.5 \\
	\hline
    Lithium-6 ($^6$Li) & 0.8 $\pm$ 0.3 & 1.0 $\pm$ 0.5 \\
    \hline
    Boron-10 ($^{10}$B) & 2.1 $\pm$ 0.3 & 2.5 $\pm$ 0.7\\
    \hline
    Beryllium-9 ($^9$Be) & 0.7 $\pm$ 0.2 & 0.9 $\pm$ 0.5 \\ 
    \hline
	\end{tabular}
	\caption{\label{tab:chi2}\(\chi^2\) Values for each charge-changing cross sections total cross-section DINo predictions compared to TENDL21 model}
\end{center}
\end{table*}

Across all tested isotopes, DINo demonstrated an ability to produce reliable predictions, although the accuracy was heavily influenced by the quality and quantity of the training data. The algorithm performed better in energy ranges with dense experimental data, indicating its potential for high accuracy in well-studied isotopes and reactions. Conversely, for isotopes with limited data, the model's predictive performance highlighted the need for more comprehensive datasets to improve accuracy.

This discussion underlines the necessity of comprehensive studies between models and measurements to enhance overall accuracy and reliability, as these factors are intricately interconnected.

\subsection{General efficiency and limits}
The evaluation of DINo's efficiency involved comparing its computational performance and predictive accuracy against the TENDL 2021 model. Key metrics included computational time, mean squared error (MSE) for predictive accuracy, and the ability to generalize predictions from training data to unseen conditions.
\subsubsection{Computational efficiency}
DINo demonstrated significant computational efficiency advantages. Once trained, the deep learning model provided rapid predictions, typically in the order of $\mu$s, requiring substantially less computational time than traditional nuclear reaction models. This speed makes DINo particularly advantageous for simulations and real-time applications, such as in clinical settings for hadron therapy planning, where quick and accurate data is crucial.
\subsubsection{Predictive accuracy}
The model's predictive accuracy was rigorously tested using cross-validation methods. DINo's predictions for total cross-sections in proton-carbon interactions were consistently more accurate, with lower MSE values, compared to TENDL, especially within the well-represented mid-energy range (10-50 MeV). However, at the extremes of the energy spectrum (below 10 MeV and above 50 MeV), the model's accuracy was more variable. This variation can be attributed to the sparse data available for training in these regions, indicating a limitation that could be mitigated with more extensive experimental datasets.
\subsubsection{Generalization capability}
One of DINo’s strengths is its ability to generalize from the training data to make predictions for unseen experimental conditions. This was particularly evident in isotopes with comprehensive datasets, where DINo provided reliable predictions even in extrapolated scenarios. However, for isotopes and energy ranges with limited experimental data, the model's generalization capability was less robust, often reflecting increased prediction variance.
\subsubsection{Limitations}
The primary limitation identified in this study is DINo's dependency on the quality and comprehensiveness of its training dataset. The algorithm performed best with isotopes and energy levels that had extensive and precise data. In contrast, its performance was less consistent for isotopes with sparse data, highlighting the need for continuous updates to the training datasets. Additionally, overfitting was observed when the training data was not sufficiently diverse, suggesting that future iterations of the model should incorporate techniques to mitigate this risk.

\section{Discussion}
